Coexistence of UAVs and Terrestrial Users in Millimeter-Wave Urban Networks

5G millimeter-wave (mmWave) cellular networks are in the early phase of commercial deployments and present a unique opportunity for robust, high-data-rate communication to unmanned aerial vehicles (UAVs). A fundamental question is whether and how mmWave networks designed for terrestrial users should be modified to serve UAVs. The paper invokes realistic cell layouts, antenna patterns, and channel models trained from extensive ray tracing data to assess the performance of various network alternatives. Importantly, the study considers the addition of dedicated uptilted rooftop-mounted cells for aerial coverage, as well as novel spectrum sharing modes between terrestrial and aerial network operators. The effect of power control and of multiuser multiple-input multiple-output are also studied.

==> 02_system_model_v1.tex <==
\section{System Model}
\label{sec:sim}

This work focuses on the uplink---the more data-hungry direction for UAVs---with the terrestrial UEs, UAVs, and BSs, all deployed in a $1 \, \text{km}^2 \times 1 \, \text{km}^2$ area with wrap-around.

\begin{table}[!t]
  \begin{center}
    \caption{Simulation parameters.}
    \label{tab:sim_params}
    \begin{tabular}{|l|l|}
    \hline
      \textbf{Parameter} & \textbf{Value}\\
      \hline
      Minimum UE-BS 2D distance (\SI{}{\meter}) &  $10$ \\
      Minimum UAV-BS 3D distance (\SI{}{\meter}) &  $10$ \\
      $\ISDs$ (\SI{}{\meter}) & $200$\\
      Height of standard BSs (\SI{}{\meter}) &  $10$\\ %Unif[2,5] 
      Height of dedicated BSs (\SI{}{\meter}) & [10,30] \\
      Bandwidth (\SI{}{\MHz}) & $400 $ \\
      Frequency (\SI{}{\GHz}) & $28 $ \\
      BS noise figure (\SI{}{\dB}) & $6$\\
      UAV height (\SI{}{\meter}) & $120$ \\
      UAV and UE maximum transmit power (\SI{}{dBm}) & $23$\\
      3GPP vertical half-power beamwidth ($\theta_{\text{3dB}}$)  & $65^\circ$\\
      3GPP horizontal half-power beamwidth ($\phi_{\text{3dB}}$) & $65^\circ$ \\
      Power control parameters, $P_0$ (\SI{}{dBm}) and $\alpha$ & -$82$, $0.8$ \\
      Number of associated users per cell & $10$\\
      \hline
    \end{tabular}
  \end{center}
  %\vspace{-5pt}
\end{table}

\subsection{Deployment and Propagation Channel Features}

\subsubsection*{Network Deployment} BSs are deployed following a homogeneous Poisson point process with a given average intersite distance (ISD), %with intensity $\lambda = \frac{4}{\pi {\rm ISD}^2}$.
and they have three sectors, each corresponding to a cell and equipped with an $8 \times 8$ uniform rectangular array (URA). 
Two types of BSs are considered: a standard deployment with antennas downtilted by $-12^\circ$, and a dedicated deployment with rooftop-mounted antennas uptilted by $45^\circ$, as illustrated in Fig.~\ref{fig:scenario}.
In turn, UAVs and terrestrial users feature $4 \times 4$ URAs. Those mounted on UAVs are downtilted by $-90^\circ$ while those at terrestrial UEs are distributed uniformly in azimuth with a fixed elevation of $0^\circ$. All the parameters are summarized in Table \ref{tab:sim_params}, following the simulation settings in~\cite{3GPP38901}. The height of dedicated BSs, which is an additional parameter, is uniformly random between $10$ and $30$ m.

\subsubsection*{UAV Radiation Pattern} In order to incorporate the effects of the UAV frame on its radiation pattern, we simulated a quarter-wave monopole antenna (with bottom hemisphere coverage) placed under the UAV and used a software package~\cite{Remcom} that utilizes geometrical optics, uniform theory of diffraction, and physical optics. %We utilize 3D laser scanned UAV model of the DJI M210 UAV in this particular XGtd simulations.
Fig.~\ref{fig:uav_antenna} illustrates the effect of the UAV on the antenna radiation pattern. The fluctuations of the antenna gain are due to protruding parts of the UAV (e.g., landing skid, gimbal) that are within the field of view of the antenna \cite{semkin2021lightweight}. Non-obviously, the effects of the UAV frame increase with the antenna directivity. We apply the obtained element radiation pattern to each UAV, whereas 3GPP antenna element patterns are adopted for BSs and UEs~\cite{3GPP37840} .

\subsubsection*{Propagation Model} The 3GPP channel model reported in~\cite{3GPP38901} is invoked to characterize the propagation between UEs and BSs (for urban microcells). To represent the mmWave propagation between UAVs and BSs, for which no calibrated model is available,
the data-driven channel model developed in \cite{XiaRanMez2020,XiaRanMez2020a} is invoked.

\begin{figure}[t!]
\centering
\includegraphics[width=0.7\columnwidth]{Figures/antenna_pattern.png}
\caption{Antenna radiation pattern accounting for the UAV frame.}
\label{fig:uav_antenna}
\vspace{-4mm}
\end{figure}

\subsection{Cell Selection and Beamforming}

Each transmitter, UE or UAV, connects to the strongest BS.
%BSs can have multiple connections with terrestrial UEs and UAVs.
%We implement SDMA to enable multiple terrestrial UEs and UAVs to simultaneously connect to each BS.
Both UAVs and UEs employ the open-loop power control policy specified in \cite{3GPP36213}. % based on the below equation. 
%\begin{equation}
    %\mathrm{P} = \mathrm{min} \{ \mathrm{P}_{max},  \mathrm{P}_0 + \alpha  \mathrm{L} + 10\log_{10} \mathrm{M}\}
%\end{equation}
With MU-MIMO, the minimum mean-square error (MMSE) receive vector for user $u$ at BS $\ell$ is given by~\cite{heath2018foundations}
\begin{align}
  \boldsymbol{w}_{\ell u} & =  \Bigg(\sum_{k=0}^{N_{\rm u}-1} \mathrm{SNR}_{\ell k} \, \boldsymbol{h}_{\ell k} \boldsymbol{h}_{\ell k}^* \nonumber \\ 
  & \quad + \Bigg(1+\sum_{n \neq \ell } \sum_{k=0}^{N_{\rm u}-1} \mathrm{SNR}_{n k} \Bigg) \boldsymbol{I} \Bigg)^{\!-1} \!\! \boldsymbol{h}_{\ell u},
\end{align}
%\angel{Should the second summation be over $n \neq \ell$?}
where $\boldsymbol{h}_{\ell k}$ and SNR$_{\ell k}$ are the channel matrix and the signal to noise ratio (SNR) between user $k$ and BS $\ell$, SNR$_{n k}$ is SNR of user $k$ in a  different cell $n$, and $N_{\rm u}$ is the number of \emph{active} users simultaneously served by one BS. %$W_{\ell u}$ is normalized by its norm so that additional powers cannot be added.} \angel{What does "so that additional powers cannot be added" mean=?}
%$\mathrm{H}^\mathrm{H}$ denotes the Hermitian matrix of H.
%\angel{All variables in math font, please.}\Seongjoon {resolved} 
As the channel matrices for other-cell users are not estimated by BS $\ell$, their interference is regarded as spatially white.

UAVs and UEs apply long-term transmit beamforming, aligning their beamforming vectors with the maximum-eigenvalue eigenvector of their channel covariance matrices~\cite{lozano2007long}. %\angel{Where is the "first hand" that precedes this "on the other hand"?}. 
Accordingly, the overall gain from user $k$ to BS $\ell$ is
\begin{equation}
    G_{\ell k} = |\boldsymbol{w}_{\ell k}^* \boldsymbol{h}_{\ell k} \boldsymbol{f}_{\ell k}|^2
\end{equation}
where $\boldsymbol{f}_{\ell k}$ is the long-term beamforming vector of user $k$. 
The interference experienced by user $u$ is then 
%\angel{Guys, this indexing is inconsistent with (1).}\Seongjoon {resolved}
\begin{align}
    I_{\ell u} & = \sum_{k \neq u} P_{\ell k}^{\mathrm{tx}} G_{\ell k}
    \sum_m{A_{\ell k m}^{\rm \mathrm{tx}} A_{\ell k m}^{\rm rx} 
    L_{\ell k m}^{-1}} \nonumber \\
    &  \quad + \sum_{n \neq \ell} \sum_{k} P_{nk}^{\mathrm {tx}}G_{n k}  
    \sum_m A_{n k m}^{\mathrm {tx}} A_{nkm}^{\mathrm {rx}} L_{n k m}^{-1},
\end{align}
%\textcolor{red}{[Suggested notation: $G_{\ell k m}$ is the path gain from,
%$W_{\ell k}$  is the beamforming gain.  Later use $F$ for the pre-coder matrix and %$B$ for the bandwidth]}
%\angel{How is $G_{n k}$ computed? This affects the issue of the out-of-cell interference being white or colored.} \Seongjoon{$G_{n k}$ is beamforming gain by sidelobes, so the cmputation is the same as equation (2).$G_{n k} = |W_{\ell u}^{*} H_{\ell k} F_{nk}|^2$ }
where $P_{\ell k}^{\mathrm{tx}}$ is the  transmit power of user $k$ in cell $\ell$, $A_{lkm}^{\mathrm{tx}}$ and $A_{lkm}^{\mathrm{rx}}$ are the transmit and receive antenna element gains on path $m$, and $L_{\ell km}$ is the pathloss along path $m$ between user $k$ and BS $\ell$. Similarly, the received power from user $u$ is
\begin{equation}
        P_{\ell u}^{\mathrm{rx}} = P_{\ell u}^{\mathrm{tx}} G_{\ell u}\sum_m{A_{\ell um}^{\mathrm{tx}} A_{\ell um}^{\mathrm{rx}} L_{\ell um}^{-1}}.
\end{equation}
Altogether, the SINR between UE $u$ and BS $\ell$ equals
\begin{align}
    \mathrm{SINR}_{\ell u} = \frac{P_{\ell u}^{\mathrm{rx}}}{I_{\ell u} +  N_0 B \,
    \|\boldsymbol{w}_{\ell u}\|^2},
\end{align}\\
where $N_0$ is the noise power spectral density and $B$ the bandwidth. %\angel{$N_0$ is the noise spectral density, not the power.}
%\angel{Since (1) is not unit-energy, the noise power must be multiplied by $\| \boldsymbol{W}_{\ell u} \|^2$}


 


==> XX_abstract_gio_note.tex <==
\quad\quad Gio's notes below --- please edit.
\newline

--- Setup:
\begin{itemize}
    \item 15 UEs per cell on average (can be PPP). A fraction of these UEs are UAVs, the rest are GUEs.
    \item Uplink communication. Important because it is the data-hungry direction for UAVs. Downlink command and control can be provided through sub-6GHz coverage umbrella.
    \item Choose the UAV height.
\end{itemize}

--- First experiment:
\begin{itemize}
    \item Only standard BSs.
    \item Spatial multiplexing (e.g., 2 users per cell).
    \item Increase the fraction of UAVs, e.g., as follows: 0/15, 1/15, 3/15, 5/15.
    \item Show SINR/rates as a function of the fraction of UAVs in the system. For the rates, account for the total number of users per cell, which is larger than the number of multiplexed users (Sundeep's formula).
    \item Message [TBC]: GUE performance degraded by the presence of UAVs. 
    \item (Optional) Effect of multiplexing more users per cell, effect of UAV height.
\end{itemize}

--- Second experiment:
\begin{itemize}
    \item Add rooftop cells progressively, e.g., with ISDs values as per SJ's conference paper. Same frequency band as standard cells.
    \item All UAVs associate to rooftop cells (either naturally or forced). All GUEs associate to standard cells.
    \item Show SINR/rates as a function of the fraction of UAVs in the system. For the rates, account for the total number of users per cell, which now is lower than in the first experiment.
    \item Message [TBC]: Total capacity increases for both GUEs and UAVs (win-win), reusing the same spectrum. 
    \item Message [TBC]: I need more dedicated cells if I have more UAVs in the system, meaning that I can slowly start deploying those until UAVs really proliferate.
    \item Message [TBC]: The reason for the performance improvement is ... (reduced UAV transmit power, higher UAV LoS probability, capacity gain due to the fact that GUEs only share capacity with GUEs since UAVs are served by dedicated cells, etc.)
\end{itemize}

--- Third experiment:
\begin{itemize}
    \item Confirm the above explanation on why rooftop cells improve performance.
    \item E.g., show CDF of the UAV transmit power for different values of the ISD of dedicated cells. E.g., does the power decrease as I deploy more dedicated cells?
    \item Does optimal power control further improve the performance? If so, provide intuition. What information does the optimal power control algorithm need? Can it be made more practical by only using partial information?
\end{itemize}

--- (Optional) Fourth experiment:
\begin{itemize}
    \item Reverse TDD: UAVs doing uplink to dedicated BSs while GUEs are doing downlink from standard BSs. Rationale: Since there are regulations against beamforming upwards, UAVs may as well use the whole time-frequency resources for their data-hungry uplink.
    \item Message {TBC]: The interference caused at the GUEs is tolerable, thanks to directionality and to the presence of rooftop BSs.}
\end{itemize}

--- List of Figures:
\begin{itemize}
    \item Illustration of system model
    \item SINR/rates vs number of UAVs. Optionally, show different number of streams per cell. Separate UAV/GUE SINR/rates?
    \item SINR/rates vs increasing density of rooftop cells, show different fraction of UAVs.
    \item Plot explaining why dedicated cells help, e.g., CDF of transmit power? Optional: optimal power control.
    \item (Optional) SINR of GUEs/UAVs under reverse TDD.
\end{itemize}


